X(3872) is not a true molecule

A solvable coordinate-space model is employed to study the $c\bar{c}$ component of the X(3872) wave function, by coupling a confined $^3P_1$ $c\bar{c}$ state to the almost unbound $S$-wave $D^0\bar{D}^{*0}$ channel via the $^3P_0$ mechanism. The two-component wave function is calculated for different values of the binding energy and the transition radius $a$, always resulting in a significant $c\bar{c}$ component. However, the long tail of the $D^0\bar{D}^{*0}$ wave function, in the case of small binding, strongly limits the $c\bar{c}$ probability, which roughly lies in the range 7-11%, for the average experimental binding energy of 0.16 MeV and $a$ between 2 and 3 GeV$^{-1}$. Furthermore, a reasonable value of 7.8 fm is obtained for the X(3872) r.m.s. radius at the latter binding energy, as well as an $S$-wave $D^0\bar{D}^{*0}$ scattering length of 11.6 fm. Finally, the $\mathcal{S}$-matrix pole trajectories as a function of coupling constant show that X(3872) can be generated either as a dynamical pole or as one connected to the bare $c\bar{c}$ confinement spectrum, depending on details of the model. From these results we conclude that X(3872) is not a genuine meson-meson molecule, nor actually any other mesonic system with non-exotic quantum numbers, due to inevitable mixing with the corresponding quark-antiquark states.

==> repair.32251.Coito.tex <==
%b This is a template file for The European Physical Journal
%
% Copy it to a new file with a new name and use it as the basis
% for your article
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{filecontents}{leer.eps}

